MobilePhys: Personalized Mobile Camera-Based Contactless Physiological Sensing

Camera-based contactless photoplethysmography refers to a set of popular techniques for contactless physiological measurement. The current state-of-the-art neural models are typically trained in a supervised manner using videos accompanied by gold standard physiological measurements. However, they often generalize poorly out-of-domain examples (i.e., videos that are unlike those in the training set). Personalizing models can help improve model generalizability, but many personalization techniques still require some gold standard data. To help alleviate this dependency, in this paper, we present a novel mobile sensing system called MobilePhys, the first mobile personalized remote physiological sensing system, that leverages both front and rear cameras on a smartphone to generate high-quality self-supervised labels for training personalized contactless camera-based PPG models. To evaluate the robustness of MobilePhys, we conducted a user study with 39 participants who completed a set of tasks under different mobile devices, lighting conditions/intensities, motion tasks, and skin types. Our results show that MobilePhys significantly outperforms the state-of-the-art on-device supervised training and few-shot adaptation methods. Through extensive user studies, we further examine how does MobilePhys perform in complex real-world settings. We envision that calibrated or personalized camera-based contactless PPG models generated from our proposed dual-camera mobile sensing system will open the door for numerous future applications such as smart mirrors, fitness and mobile health applications.

==> revisions/major.tex <==
\subsection*{Major Revisions}
\label{sec:revisions-major}

\begin{enumerate}[labelsep=6mm,label=(MJ-\arabic*)]

\item \reviewcomment{
\textbf{Novelty and Contribution}
~\\
\textbf{AE1:} “Justify the technical novelty of the work.”
~\\

\textbf{AE1:} “In one specific place in the paper, provide a very streamlined and precise description of the relative advantages of this method against its nearest methods (i.e., other meta-learned based PPG vision approaches). A table with advantages and disadvantages would likely help.” 
~\\

\textbf{AE2:} "Provide experiments that compare to the degree possible with the very closely related other techniques -- some of which are being built ontop of (e.g., MetaPhys). And where not possible, turn qualitative arguments as to why this method is better into quantative ones."
~\\

\textbf{AE2:} “However my hesitation in accepting the work in its current form largely stems from the series of works it builds on, and especially MetaPhys. ... I feel additional comparisons and contrasting are needed. Meta-rPPG and MetaPhys as the authors pointed out ...”
~\\

\textbf{R5:} “The major contribution I was excited about is the meta-learner and the ability to leverage the low density data for personalizing the system. However, it looks like this has been already presented in MetaPhys and it seems that there is a significant overlap between MetaPhys and MobilePhys. Please revisit your contribution section and clearly define how you are building on top of MetaPhys (https://arxiv.org/abs/2010.01773)."
~\\
}

To better demonstrate the novelty and contributions of our work, we significantly improved and revised the evaluation of this paper. To summarize our changes: 1) we recruited 15 new subjects with different skin types under different lighting conditions and motion tasks using a new mobile device - iPhone 11. By complementing this new dataset, \projectname is evaluated in 39 subjects, 3 motion tasks, 3 lighting conditions, 3 lighting intensities, 3 skin types (Fitzpatrick scale: I+II, III+IV, V+VI), 2 smartphone devices with different operating systems (Xiaomi 8 and iPhone 11). 2) We added the performance comparison between \projectname and MetaPhys to demonstrate the benefits of our proposed method. We would also like to emphasize that MetaPhys was only proposed and evaluated on two public datasets with stationary tasks and were recorded by high-end professional cameras. On the other hand, \projectname was proposed and evaluated on diverse real-world mobile settings ranging from lighting, motion, and skin types. Through the results on Table~\ref{tab:result_motion_task} to \ref{tab:lighting_level_table}, MetaPhys did not generalize as well on real-world mobile camera settings, while \projectname still achieves superior performance compared to the cutting-edge supervised method.  \\


The technical novelties and contributions of \projectname include 1) we propose a novel dual camera-based mobile physiological sensing system that leverages the back/rear camera to generate high-quality pseudo PPG labels for few-shot adaptation and personalization. 2) Through comprehensive user studies and evaluation, we demonstrate \projectname can generalize to various real-world conditions with different motion tasks, lighting conditions/intensities, and subject skin types. 3) we compare our proposed system \projectname with the state-of-the-art on-device few-shot adaptation method, MetaPhys, and demonstrate our system consistently outperforms our baseline in all scenarios. 4) we also study and investigate mobile camera settings, which we believe will be valuable for guiding future research in mobile physiological sensing. 
%to explore an optimal setting in contactless camera-based physiological sensing to capture subtle pixel changes

~\\

\item \reviewcomment{
\textbf{Effectiveness in Real-world Setups}
~\\
~\\
\textbf{AE1:} “Provide more experiments and evaluations in real-world setups such as deploying the personalized model on different devices and showing its effectiveness and contrasting experiments to show the benefit of current work compared to close prior research.”
~\\

\textbf{R4:} “In the introduction, the authors claim, "This customized or personalized model from MobilePhys could then be deployed on the phone or shared with other smart devices..." However, the authors do little to back this claim. I would encourage the authors to *actually* deploy the personalized model on different devices and show its effectiveness. Given the camera quality varies greatly from device to device, won't it require some form of calibration or color correction for each new device?”
~\\

\textbf{R4:} “I would also request the authors consider other scenarios, like dim lighting conditions, different smartphones, when participants are doing basic tasks, like typing.”
~\\

\textbf{R4:} “I am concerned about the incremental technical novelty -- the authors mostly leverage prior works, methods, and models in their work, with the new contribution being the meta-learning model -- and the lack of a thorough evaluation, with only 24 participants and 14 minutes worth of data per participant in a handful of different conditions, using only one smartphone. Given the several strong claims in the paper, I was hoping for a more detailed evaluation."
~\\

}

In this revision, we added new experiments to show the effectiveness of \projectname under a range of conditions and demonstrate its benefits compared to MetaPhys/TS-CAN, which is the closest prior research. In Table~\ref{tab:result_motion_task} to \ref{tab:lighting_level_table}, we empirically show that \projectname consistently outperforms MetaPhys regarding motions, lighting conditions, lighting intensities, and skin types, as summarized in section~\ref{sec:result}.  Moreover, we would like to point out MetaPhys is the only published work demonstrating mobile on-device personalization. Meta-rPPG uses a synthetic gradient generator and a prototypical distance minimizer to perform transductive inference to enable self-supervised meta-learning. This method is not specifically designed for personalization, and its processes require a significant computational budget and are not suited to mobile platforms. In this project, our core claim is to enable personalized \textbf{mobile} camera-based contactless physiological sensing. \\


To better support our claim about ``This customized or personalized model from MobilePhys could then be deployed on the phone or shared with other smart devices...", we conducted an additional experiment with 15 new subjects using an iPhone 11. In this experiment, we used the same camera settings as in our previous experiments (Android Xiaomi 8). As Table~\ref{tab:result_motion_task} to \ref{tab:lighting_table} illustrated, \projectname achieves superior performance in both mobile platforms. \\

In Table~\ref{tab:skin_tone_table} and \ref{tab:lighting_level_table}, we also add evaluation of how \projectname works in different lighting intensities (dimmer light) and skin types. Again, \projectname achieved strong improvement compared to the baseline methods. \\

\\
\item \reviewcomment{
\textbf{Choice on the Baseline Method}
~\\
~\\
\textbf{AE1:} “Justify the choice of comparison methods and leaving out other similar methods.”

~\\

\textbf{R4:} “It is unclear why the authors chose to compare with TS-CAN and not other models like Hyb-CAN or 3D-CAN from the same paper [1]. I would urge the authors to conduct additional experiments to test this.”
~\\
}

Our goal was to propose a mobile physiological sensing system, therefore using models that run on-device is important. To the best of our knowledge, TS-CAN~\cite{liu2020multi} and MetaPhys~\cite{liu2021metaphys} are the best baseline papers that focus on on-device camera-based physiological sensing. Therefore, we chose TS-CAN and MetaPhys as our baselines. \\

% THIS IS JUST A REPETITION OF THE ABOVE
%Moreover, 3D-CAN and Hybrid-CAN are to computationally have to enable real-time inference on mobile platforms, especially for these low-end smartphones. Moreover, we would also like argue that our proposed dual-camera penalization system should be plug-in-play and applicable to any type of network because it can yield high-quality self-supervised labels which are not device specific. 


\vspace{0.5cm}


\item \reviewcomment{

\textbf{Clarification on Experiment Setups and Results}
~\\
~\\

\textbf{AE1:} “Clarify and discuss the evaluation setups and provide performance results in different settings.”
~\\

\textbf{R4:} "In section 5.2, the authors mention that MetaPhys needed only 18 seconds of data to train the personalized model. Is it 18 seconds just at the beginning of the study (i.e., 18 seconds out of the 14 minutes per user), or 18 seconds for each task? Is it possible that the ordering of the tasks might affect it? From the evaluations, it seems that TS-CAN performs similar to MobilePhys in incandescent and LED lighting but very poorly in Natural lighting conditions. Could this be because TS-CAN training data doesn't have any data in natural lighting conditions, whereas MobilePhys does? "

~\\

\textbf{R4:} “I request the authors to please report the actual results and values about MobiPhys' performance when the participants were exercising along with the relative improvements over TS-CAN.”

~\\

\textbf{R5:} “Authors state that users are required to calibrate the system for only 18sec. How is this calibration phase impacted by lighting conditions? Do users need to calibrate the system in different lighting levels (e.g., indoor vs. outdoor)?”

~\\

\textbf{R5:} “Were there any variations in the performance of this approach based on skin tone, gender, or other demographics? Authors should consider discussing this in the paper."

~\\

}

For \projectname to generate a personalized model, it requires \textbf{18 seconds video of each task}. For a fair comparison, the TS-CAN model fine-tuned on the same 18-second segments of video. Therefore, TS-CAN had access to the same data as \projectname during the training phase and had samples with all lighting conditions. However, with such small amounts of data to fine tune, a traditional supervised model does not perform well. \\ 

% THIS SENTENCE BELOW DOESN'T REALLY MAKE SENSE TO ME:
%Moreover, we would also like to argue that natural light has a very wide spectrum, therefore there is no way to include all the entire spectrum of natural light in the training dataset. Therefore, a self-supervised adaptation is needed during real-world deployments.\\ 

We apologize that this was not clear. We did report performance for the models when the participants were exercising in Table \ref{tab:exercise_table}. We have updated the table caption to help readers to easier to find it. \\

To better respond to R5's question, we have added the results of new experiments to demonstrate the proposed \projectname generalizes well to different skin types and lighting conditions and levels.   \\








\item \reviewcomment{
\textbf{Discussion, Limitations, and Future Work}
~\\
~\\
\textbf{AE1:} “Discuss the limitations of the work.”
~\\

\textbf{AE1:} “Expand the discussion of the results and findings rather than just summarizing them.”
~\\

\textbf{R3:} “The discussions need to be more concrete in justifying the results.”
~\\

\textbf{R5:} “The authors claim that this method is robust to noise and motion artifacts. However, the camera was fixed in the experiment. This is very unlikely to happen in real word applications, especially the ones using smartphones. It looks like authors focused on head motion only, and assumed that the camera would be fixed. This seems to be a major limitation and needs to be better discussed in the paper.”

~\\

}

Thanks for the feedback. In the revised version, we added a limitations section and expanded the discussion section to discuss our findings and justify our results. We also included that the phone was fixed as a limitation, as R5 pointed out. 

\end{enumerate}

==> revisions/minor.tex <==
\subsection*{Minor Revisions}
\label{sec:revisions-minor}

\begin{enumerate}[labelsep=6mm,label=(MN-\arabic*)]

\item \reviewcomment{
\textbf{R3:} “With respect to figure 6 the authors mention in discussion that there is "descent improvement in waveform quality" but this not clear from the figure what markers are the readers suppose to look for in the figure to establish this.”
~\\
}
\item \reviewcomment{
\textbf{R4:} “I am unsure what to make of Fig 6. I would request the authors to please explain the figure in the text.”
~\\
}

Due to the new results and experiments added during this revision cycle, we decided to remove Figure 6 to make sure that our results are not overwhelming and not distract readers' attention. Moreover, this paper is focused on quantitative results (e.g., heart rate), not qualitative results (e.g., morphology). Figure 5 (bar plot) was also removed as we believe we already covered all the results in Table 4-8. \\


\item \reviewcomment{
\textbf{R4:} “Further, as the authors expect their system to run on the users' smartphones, what are the battery life considerations that need to be made? Somewhere in the text, the authors mentioned phone overheating, so I am concerned about the actual deployability.”
~\\
}

We did not evaluate battery life in this paper because we believe 18-seconds video personalization would have a limited, almost negligible, impact on the battery life. The phone over-heating only happened during the data collection as the mobile device was continuously used for recording for a few hours. In practice, a recording would not be necessary as frames would be processed ``on-the-fly''. We will add this point to future work. \\

\item \reviewcomment{
\textbf{R5:} “Most recent phones come with multiple rear cameras, how does MobilePhys handle this?”
~\\
}

\projectname is a RGB-camera based solution, but exploring other cameras such as true-depth or IR camera is an interesting direction. As we listed in the future work, we will open-source our dataset and continue exploring this direction.  \\

\item \reviewcomment{
\textbf{R5:} “There are numerous places with bad English. Examples include but not limited to:
 "Building on this, we examine which source of noise personalization helps adapt to best".
"First, there is still a accuracy gap."....etc.”
~\\
}

We apologize for these grammar mistakes and updated the text to fix these language issues. \\

\end{enumerate}

==> revisions/overall.tex <==
\section*{Review Responses}
We would like to thank the reviewers for their detailed, valuable and constructive feedback on our work. We have used this revision cycle as an opportunity to improve our article. The most significant changes involve the paper's stated contributions and the validation of effectiveness in real-world settings. We have added an additional user study to evaluate our method's effectiveness across devices, lighting conditions, and skin types as AE1, AE2, and R4 suggested. Furthermore, we evaluated our method's performance when compared with related techniques (MetaPhys and TS-CAN) under various conditions as AE1, AE2 and R5 suggested. Our method performs well in comparison. Finally, we clarify our unique contributions when compared with state-of-the-art camera physiological sensing methods. \\

Because of the significant changes and additional results in this revision cycle, we removed Figure 5 and 6 to ensure we can clearly deliver our core contributions. We also modified Table \ref{tab:data_collection} and Table \ref{tab:overall_subjs} to better reflect the new combined dataset. The details are discussed in the major revision section as well. \\

In the following document, we have provided detailed responses to each of the suggestions, concerns, and questions raised by the reviewers.
The reviewers' comments are in boxes, and our responses to each comment follow. Reviewer remarks are grouped to avoid redundancy.
Changes within the revised article itself are marked in red text.\\

Our responses are structured as follows:
\begin{itemize}
\item Major revisions: Page~\pageref{sec:revisions-major}
\item Minor revisions: Page~\pageref{sec:revisions-minor}
\end{itemize}

